Cross-Domain Image Manipulation by Demonstration

In this work we propose a model that can manipulate individual visual attributes of objects in a real scene using examples of how respective attribute manipulations affect the output of a simulation. As an example, we train our model to manipulate the expression of a human face using nonphotorealistic 3D renders of a face with varied expression. Our model manages to preserve all other visual attributes of a real face, such as head orientation, even though this and other attributes are not labeled in either real or synthetic domain. Since our model learns to manipulate a specific property in isolation using only "synthetic demonstrations" of such manipulations without explicitly provided labels, it can be applied to shape, texture, lighting, and other properties that are difficult to measure or represent as real-valued vectors. We measure the degree to which our model preserves other attributes of a real image when a single specific attribute is manipulated. We use digit datasets to analyze how discrepancy in attribute distributions affects the performance of our model, and demonstrate results in a far more difficult setting: learning to manipulate real human faces using nonphotorealistic 3D renders.

==> 00TODO.tex <==
+ add table with quantitative results on digits
+ new Figure 1, move existing to later pages as an example

+ describe quantitative results
+ describe implementation
+ different digit dataset

- run quantitative eval on faces: 
    * train a mouth and orientation detector in target
    - train mouth and orientation detector in source
    - change eval code to use these networks and props
- run qualitative test on lighting, skin tone, skull shape: generate: 
    + domain: 
    - domain: skull, vary: skin, expr, lighing?
    - domain: skull, vary: skin, expr

- add related work
- add more pictures with faces (including all syn2syn)

? add other metrics to digits (other r-ij) - not really, size is not present in rotation dataset

